Averages of b-hadron properties at the end of 2006

This article reports the world averages for measurements on b-hadron properties obtained by the Heavy Flavor Averaging Group (HFAG) using the available results at the end of 2006. In the averaging, the input parameters used in the various analyses are adjusted (rescaled) to common values, and all known correlations are taken into account. The averages include lifetimes, neutral meson mixing parameters, parameters of semileptonic decays, branching fractions of B decays to final states with open charm, charmonium and no charm, and measurements related to CP asymmetries.

==> b2charm_summer2006_v009/b2charm_summer2006_v009.tex <==
\input{b2charm_summer2006_v009_preamble.tex} 
\input{b2charm_summer2006_v009_symbols.tex} 

\begin{document} 
\input{b2charm_summer2006_v009_blurb.tex} 
\clearpage 
\input{b2charm_summer2006_v009_tables.tex} 
\end{document} 



